Decentralized convex optimization under affine constraints for power systems control

Modern power systems are now in continuous process of massive changes. Increased penetration of distributed generation, usage of energy storage and controllable demand require introduction of a new control paradigm that does not rely on massive information exchange required by centralized approaches. Distributed algorithms can rely only on limited information from neighbours to obtain an optimal solution for various optimization problems, such as optimal power flow, unit commitment etc. As a generalization of these problems we consider the problem of decentralized minimization of the smooth and convex partially separable function $f = \sum_{k=1}^l f^k(x^k,\tilde x)$ under the coupled $\sum_{k=1}^l (A^k x^k - b^k) \leq 0$ and the shared $\tilde{A} \tilde{x} - \tilde{b} \leq 0$ affine constraints, where the information about $A^k$ and $b^k$ is only available for the $k$-th node of the computational network. One way to handle the coupled constraints in a distributed manner is to rewrite them in a distributed-friendly form using the Laplace matrix of the communication graph and auxiliary variables (Khamisov, CDC, 2017). Instead of using this method we reformulate the constrained optimization problem as a saddle point problem (SPP) and utilize the consensus constraint technique to make it distributed-friendly. Then we provide a complexity analysis for state-of-the-art SPP solving algorithms applied to this SPP.

==> dump.tex <==
The regularization allows us to derive the convergence by distance to saddle point from the convergence by duality gap.
Let $h(x,y)$ be an arbitrary $\mu$-strongly-convex-strongly-concave function (enough for existence of sp?, on what set?). Then for duality gap we write 
\begin{multline}
\eps_{gap}(x_N, y_N) = \sup_y h(x_N, y) - \inf_x h(x, y_N)
= \overline{h}(x_N) - \underline{h}(y_N) \\ 
= \left(\overline{h}(x_N) - \overline{h}(x_*)\right)  
+  \left(\underline{h}(y_*) - \underline{h}(y_N)\right) 
= \eps_{\overline{h}}(x_N) + \eps_{\underline{h}}(y_N),
\end{multline}
where $\overline{h}(x)$  and $\underline{h}(y)$ are $\mu$-strongly-convex and  $\mu$-strongly-concave respectively.
% If $\eps_{gap}(x_N, y_N) \leq \eps$ then $eps_{\overline{f}}(x_N) \leq \eps$. 
From strong convexity of $\overline{h}(x)$ we have
$\eps_{\overline{h}}(x_N) \geq \frac{1}{2}\mu\|x_N - x_*\|^2$ and therefore 

\begin{equation}
    \|x_N - x_*\|^2 \leq \frac{2}{\mu} \eps_{gap}(x_N, y_N). 
\end{equation}

One can easily incorporate inequalities \eqref{eq:cp:p:ic} into this analysis by substituting
\begin{equation}
y \to \begin{pmatrix} y \\ z \end{pmatrix},~
A \to \begin{bmatrix} A \\ C \end{bmatrix},~
\sY \to \sY \times \R^h_+ .
\end{equation} 

\textbf{Common variables}

To handle common-variables generalization of the problem given by \eqref{eq:cpc:p}
in a decentralized manner we have to blow-up vector of common variables
and introduce usual consensus constraint via blowed-up Laplace matrix:

\begin{equation}
     \tbx = (\tx^{1\top},\dots,\tx^{l\top})^\top,~
     \tmW\tbx = 0,
\end{equation}

And since it implies that
$\tx^1 = \ldots = \tx^l$,
constraint 
$\tA \tx + \tb = 0$
could be rewritten in numerous ways, e.g. in following equivalent systems of linear equations:
$$\tA \tx^1 + \tb = 0, \text{ or}$$
$$\tA^{i1}  \tx^{11} + \tA^{i2}  \tx^{22} + \ldots = b^i~ \forall i,$$
or in the most redundant way

$$
\tmA_* \tbx + \tilde \bb = 0
$$
where

\begin{equation}
\begin{gathered}
    \tmA_* = \diag(\tA,\dots,\tA), 
    \tilde\bb = (\tb^{\top},\dots,\tb^{\top})^\top.\\
    % \mC = \diag(C^1,\dots,C^l), \bd = (d^{1\top},\dots,d^{l\top})^\top,\\
\end{gathered}
\end{equation}

Let us denote $\tmA $ any matrix such that systems
\begin{equation*}
     \tmW \tbx = 0,~
\tmA \tbx + \tilde\bb = 0
\end{equation*}
and
\begin{equation*}
     \tmW \tbx = 0,~
\tmA_* \tbx + \tilde\bb = 0
\end{equation*}
are equivalent.

Then Lagrangian for distributed reformulation of problem \eqref{eq:cpc:p} would be
\begin{equation}\label{eq:sf_l_full}
    L = \sum_{k=1}^l f^k(x^k, \tx^k)
    + \by^{\top} \left(\mA\bx + \bb\right) + \bz^\top \mW \by
    + \tby^\top \left(\tmA \tbx + \tilde\bb \right)
    + \tbz^\top \tmW \tbx ,
\end{equation}

and the saddle point problem is
\begin{equation}\label{eq:sf_sp_full}
\min_{\bx, \tbx, \bz} \max_{\by, \tby, \tbz} 
L(\bx, \tbx, \by, \tby, \bz, \tbz).
\end{equation}



Using   we acquire complexity estimate w.r.t duality gap for Mirror-Prox algorithm applied to the problem \eqref{eq:sf-sp:d}:
\begin{equation}
    N = O\left(
    \max_{k\in \{1, \ldots, l \}} \{L_k, \sigma^2_{max}(A_k), \gamma \lambda_{max}(\mW)\}
    \left( (R_x^2 + R_y^2) + 
    \frac{M_y^2}{ \left(\gamma \lambda^+_{min}(\mW)\right)^2}
    \right)
    \cdot \frac{1}{\eps} \right).
\end{equation}



While this provides us complexity estimate w.r.t. duality gap as a natural suboptimality measure for the saddle-point problem, 
our original goal was to solve the minimization problem.
Therefore it is essential to analyze convergence of our method in terms of accuracy $\eps$ of the solution to the initial problem given by
\begin{equation*}
    f(\bx_N) - f(\bx_*) \leq \eps.
\end{equation*}

To do that we regularize the Lagrangian to make it $\mu$-stongly-convex-strongly-concave:
\begin{equation}
    L'(\bx, \by, \bz) = L(\bx, \by, \bz) 
    + \frac{\mu }{2} \left(
        \|\bx\|^2 - \|\by\|^2 + \|\bz\|^2
    \right),
\end{equation}
where $\mu_x = $.

